Strategic Ranking

Strategic classification studies the design of a classifier robust to the manipulation of input by strategic individuals. However, the existing literature does not consider the effect of competition among individuals as induced by the algorithm design. Motivated by constrained allocation settings such as college admissions, we introduce strategic ranking, in which the (designed) individual reward depends on an applicant's post-effort rank in a measurement of interest. Our results illustrate how competition among applicants affects the resulting equilibria and model insights. We analyze how various ranking reward designs, belonging to a family of step functions, trade off applicant, school, and societal utility, as well as how ranking design counters inequities arising from disparate access to resources. In particular, we find that randomization in the reward design can mitigate two measures of disparate impact, welfare gap and access.

==> old_material.tex <==

\section{Old material}

\begin{example}[Fuzzy rank with unmeasurable skill]\label{ex:2skills}
\begin{itemize}
    \item College has capacity for $\rho$ mass of students. Admission policy is to take the top $\lambda > \rho$ fraction of students in terms of test score (all students above an `initial cutoff score', denoted $s_0$), and of those each is accepted with probability $\frac{\rho}{\lambda}$.
    \item Student has potential $(\theta^M, \theta^U)$ for the measurable and unmeasurable skill respectively (e.g. testing and creativity). They distributed, independently, according to CDFs, $\Theta^M(\cdot)$ and $\Theta^U(\cdot)$ respectively.
    \item Students have a fixed effort budget of $1$. They can exert effort $(e^M, e^U)$ where $e^M +e^U =1$ to obtain results $(s^M, s^U) = (\theta^M\cdot e^M,\theta^U\cdot e^U) $, where only $s^M$ is observable (e.g. a test score). Subject to their effort budget, students maximize total welfare:

    \begin{equation}
        W(e) =  u \cdot \frac{\rho}{\lambda} \cdot \Ind{s^M \text{ is in top }\lambda} - (e^M-\tilde{e}^M)^2,
    \end{equation}
    where $\tilde{e}^M$ is the preferred or `natural' effort level for testing.

    As aforementioned, we assume that whatever effort that is not spent on testing is spent on creativity, i.e. $e^U = 1-e^M$, if $e^M < 1$.
    \item Admission outcome for each student $Z$ is denoted $Z \in \{0,1\}$.

    The college's objective to maximize the joint skill of the admitted class weighted by $\alpha$:
    \begin{equation}
        U = \E[\alpha\cdot s^M + (1-\alpha)s^U\mid Z=1].
    \end{equation}
\end{itemize}
\end{example}

We can characterize the equilibrium for Example~\ref{ex:2skills} as follows:
\begin{itemize}
\item Denote $\theta^M_{1-\lambda}:=(\Theta^M)^{-1}(1-\lambda)$. To simplify the evaluation of the equilibrium score cutoff, we assume that $\tilde{e}^M$ is a fixed value that is the same for all students.

% , and that \begin{equation}\label{eq:assump-effort}
%     \tilde{e}^M < \frac{\theta^M_{1-\lambda}}{1-\theta^M_{1-\lambda}}\sqrt{u \cdot \frac{\rho}{\lambda}}
% \end{equation}
    \item Initial cutoff score is \begin{equation}
        s_0 = \theta^M_{1-\lambda}\cdot\left(\sqrt{u \cdot \frac{\rho}{\lambda}} + \tilde{e}^M \right).
    \end{equation}
    \begin{proof}
    For $s_0$ to be an equilibrium cutoff, only a $\lambda$ fraction of the student population can gain a non-negative expected payoff by earning test score $s_0$ or higher, that is,
    \begin{equation}\label{eq:opt-cond}
        \exists s \ge s_0 :~ u \cdot \frac{\rho}{\lambda} \ge (\frac{s}{\theta^M} - \tilde{e}^M)^2.
    \end{equation}
   We may check that equation~\eqref{eq:opt-cond} is true if and only if $\theta^M \ge \theta^M_{1-\lambda}$. First, for $\theta^M < \theta^M_{1-\lambda}$, we have
   \begin{align*}
      \frac{s_0}{\theta^M} = \frac{\theta^M_{1-\lambda}}{\theta^M} \left(\sqrt{u \cdot \frac{\rho}{\lambda}} + \tilde{e}^M \right) &> \sqrt{u \cdot \frac{\rho}{\lambda}} + \tilde{e}^M \\
      \implies u \cdot \frac{\rho}{\lambda} &< (\frac{s}{\theta^M} - \tilde{e}^M)^2.
   \end{align*}
   Now, for $\theta^M \ge \theta^M_{1-\lambda}$, we first note that for $\theta^M > \frac{s_0}{\tilde{e}^M}$, the student can get a strictly positive payoff by earning test score $s =\theta^M \cdot \tilde{e}^M > s_0$. For $\theta^M  \le \frac{s_0}{\tilde{e}^M}$, we have:
   \begin{align*}
    \frac{s_0}{\theta^M} = \frac{\theta^M_{1-\lambda}}{\theta^M} \left(\sqrt{u \cdot \frac{\rho}{\lambda}} + \teM \right) &\le \sqrt{u \cdot \frac{\rho}{\lambda}} + \tilde{e}^M \text{ and }\frac{s_0}{\theta^M} - \teM \ge 0 \\
     \implies    u \cdot \frac{\rho}{\lambda} &\ge (\frac{s_0}{\theta^M} - \tilde{e}^M)^2.
   \end{align*}
    \end{proof}
    \item Student's equilibrium effort. A student with $\theta^M$ exerts effort
    \begin{equation}
        e^M = \begin{cases}
    \frac{s_0}{\theta^M} &\text{ if } \theta^M_{1-\lambda} \le \theta^M \le \frac{s_0}{\teM}\\
    \tilde{e}^M &\text{ o.w.}
    \end{cases}
    \end{equation}
    \item We may compute the overall welfare of the student population as follows:
    \begin{align*}
        \E_{\theta \sim \Theta}[W] &= \int_{\Theta^{-1}(1-\lambda)}^{\Theta^{-1}(1)}u \cdot \frac{\rho}{\lambda} - \left(\frac{s_0}{\theta} - \teM\right)^2 d\theta
    \end{align*}
    \lnote{tbc}

    \item \textbf{The school's utility given $\lambda$.} Denote $I_\lambda:=(\potMlambda,\frac{s_0}{\teM})$. We have
    \begin{align*}
        U &= \frac{U_1\cdot\Pr(\theta^M \in I_\lambda)+U_2\cdot \Pr(\potM > \frac{s_0}{\teM})}{\Pr(\theta^M \ge \potMlambda)},
    \end{align*}
    where $U_1=\E\left[\alpha\cdot s_0 + (1-\alpha)\theta^U\left(1-\frac{s_0}{\theta_M}\right)\mid \theta^M \in I_\lambda \right]$ and $U_2 = \E\left[ \alpha \teM\potM + (1-\alpha)\theta^U(1-\teM)\mid \potM > \frac{s_0}{\teM} \right]$. Using the independence of $\theta^U$ and $\theta^M$ we may simplify:
    \begin{align*}
        U_1 &=\alpha\cdot s_0 + (1-\alpha)\E\left[ \theta^U \right] + (1-\alpha) s_0\E\left[\frac{\theta^U}{\theta_M} \mid \theta^M \in I_\lambda \right]\\
        U_2 &= \alpha\cdot \teM\E\left[\potM\mid\potM > \frac{s_0}{\teM}\right] + (1-\alpha)\cdot(1-\teM) \E[\theta^U]
    \end{align*}
    We also have
    \begin{align*}
        \E\left[\frac{\theta^U}{\theta_M} \mid \theta^M \in I_\lambda \right]\Pr(\theta^M \in I_\lambda) &= \left[ \frac{1}{2}\log y \right]^{\potMlambda}_{s_0/\teM}
    \end{align*}
    \lnote{Taking derivative with respect to $\lambda$ seems nasty. Another approach to reason whether the school's utility is maximized by a particular $\lambda$, e.g. more general setting, well-behaved distributions?}
\end{itemize}

 %\lnote{For reference: alternative welfare formulations to encode internal motivation e.g. \begin{equation}
    %     W(e) = u \cdot \frac{\rho}{\lambda} \cdot \Ind{s^M \text{ is in top }\lambda} + \beta\cdot s^M + (1-\beta)s^U - (e^U+e^M)^2, or
    % \end{equation}
    % \begin{equation}
    %     W(e) = u \cdot \frac{\rho}{\lambda} \cdot \Ind{s^M \text{ is in top }\lambda} + \beta\cdot s^M + (1-\beta)s^U \text{ where }  e^M +e^U =1
    % \end{equation}}

\begin{example}[Fuzzy rank]
\begin{itemize}
    \item College has capacity for $\rho$ mass of students. Admission policy is to take the top $\lambda > \rho$ fraction of students in terms of test score (all students above an `initial cutoff score', denoted $s_0$), and of those each is accepted with probability $\frac{\rho}{\lambda}$.
    \item Student with ability $\theta$ can exert effort $e$ to obtain test score $s=\theta \cdot e$. Utility of being admitted to college is $u$. $C(e) = e^2$ denotes the cost of effort. Student's total welfare for exerting effort $e$:
    \begin{equation}
        W(e) = u \cdot \frac{\rho}{\lambda} \cdot \Ind{\theta \cdot e \text{ is in top }\lambda} - C(e)
    \end{equation}
    \item Students have ability $\theta$ distributed according to CDF,  $\Theta(\cdot)$. The quantile function for ability is denoted $\Theta^{-1}(\cdot)$.
\end{itemize}
We can characterize the equilibrium as follows:
\begin{itemize}
    \item Initial cutoff score is \[  s_0 = \Theta^{-1}(1-\lambda)\sqrt{u \cdot \frac{\rho}{\lambda}}  \]
    \item The top $\lambda$ fraction of students in terms of ability earn score $s_0$ and have expected welfare:
    \[  W = u \cdot \frac{\rho}{\lambda} - \left(\frac{s_0}{\theta}\right)^2 \]
    \item The rest of the students earn score $0$ and have expected welfare $0$.
    \item We may compute the overall welfare of the student population as follows:
    \begin{align*}
        \E_{\theta \sim \Theta}[W] &= \int_{\Theta^{-1}(1-\lambda)}^{\Theta^{-1}(1)}u \cdot \frac{\rho}{\lambda} - \left(\frac{s_0}{\theta}\right)^2 d\theta \\
        &=u \cdot \frac{\rho}{\lambda} \left( \Theta^{-1}(1) - \Theta^{-1}(1-\lambda)+\frac{(\Theta^{-1}(1-\lambda))^2}{\Theta^{-1}(1) } -  \frac{(\Theta^{-1}(1-\lambda))^2}{\Theta^{-1}(1-\lambda) } \right)
    \end{align*}
    \item Assuming uniform $[0,1]$ distributed ability, we can simplify:
    \begin{align*}
        \E_{\theta \sim \Theta}[W] &= u \cdot \frac{\rho}{\lambda} \left(  \lambda + (1-\lambda)^2 - (1-\lambda) \right) \\
        &=u\cdot \rho \cdot \lambda
    \end{align*}
    Somewhat surprisingly, the students' overall welfare increases with $\lambda$ in this case.
\end{itemize}
\end{example}


General effort model:
\begin{itemize}
    \item $K$ metrics of student performance, e.g. SAT, APs, extra-curriculars: $i \in \{1, \cdots, K\}$
    \item Student ability corresponding to metric $i$ (relevant characteristic): $r_i$
    \item Student environment factor corresponding to metric $i$ (irrelevant characteristic): $b_i$
    \item Student's chosen effort level for each metric: $e_i$
    \item Performance in each metric: \[p_i = b_i\cdot r_i \cdot \sqrt{e_i}\]
    \item Cost of effort: $c(e_1, \cdots, e_K) = (e_1+\cdots+e_K)^2$. Think of this as the cost of time.

    \item Admissions criteria: Student is admitted with probability proportional to \[ \sum_{i=1}^K \alpha_i p_i \]
    $\alpha_i$ is the relative weight of metric $i$ in the admissions decision.
    \item Student chooses effort by optimizing own welfare gains, which is probability of admission minus cost of effort:
    \[W(e) = \sum_{i=1}^K \alpha_i p_i - c(e_1, \cdots, e_K) \]
\end{itemize}

\begin{proposition}
Consider 2 student types: $\A$ and $\B$. Type $\A$ students and Type $\B$ students have the same ability for every metric, but Type $\B$ is disadvantaged in terms of environment factors: \[ b_i^\A \geq b_i^\B \]

Informal statement: Admissions criteria $\alpha$ improves ...
\end{proposition}



Research questions:
\begin{enumerate}
    \item When does down-weighting or removing a metric increase the welfare of type $\B$ students / reduce the welfare gap?
    \begin{itemize}
        \item It depends which metrics the weight is reallocated to and in what way.
        \item \lnote{Even in the 2 metrics case the closed form solution for $e^*$ (and $W^*$) is quite unwieldy: \[ e^*_2 = \left( \frac{\alpha_2b_2r_2}{4(\lambda^2+1)} \right), \lambda := \frac{\alpha_1b_1r_1}{\alpha_2b_2r_2}\]}
    \end{itemize}
    \item Admissions criteria that maximizes welfare? \lnote{Not sure what's a good real-life analogue for this?}
    \item Observation: students with different environment factors but the same abilities will not be choosing the same effort vector.
    \lnote{I think there's another potential point here about the difficulty of equalizing opportunity: to incentivize students to choose the same effort regardless of their environment, you need to know how environment $b$ changes the score $p$ at every $e$ and $r$.}
\end{enumerate}

\section{Surveying models in education and admissions}

\begin{itemize}
    \item Modelling the school's objective(s)
    \begin{itemize}
        \item Academic Merit
        \begin{itemize}
            \item E.g. school's objective is classification accuracy (classifying ``qualified" and ``unqualified" students)
        \end{itemize}
        \item Diversity
    \end{itemize}
\end{itemize}

Section 4.2 of recent ML/MD survey (Finocchiaro et al 2021) \url{https://web.stanford.edu/~monachou/fairMLMD.pdf}

\section{Future achievement model}

\paragraph{Motivation} Machine learning models have been used in graduate school admissions, such as GRADE at University of Texas Austin \citep{waters2013grade}, to much public chagrin. One criticism is that the ML model is trained to replicate the admissions committee's decisions in the past, and is hence doomed to replicate their mistakes and biases in future decision-making.

A important question to ask is: if one were to design an admissions procedure from first principles, what are the desiderata (e.g. successful researchers at graduation, equality of opportunity, diversity of class), and what are the trade-offs between them?

If the admissions committee were to admit students based only on future success, how well does this policy align with other goals, like equality of opportunity, given existing levels of inequality in previous educational opportunities?

\begin{example}[Future achievement]
We consider the future achievement model defined as follows:
\begin{align}
    \sc &= \sn+ \ec\cdot p \tag{current skill} \\
    \sg &= \sc+ \eg \cdot p \tag{future skill}
\end{align}

Suppose
\begin{itemize}
    \item $\sn$ for all students is 1.
    \item the ability to improve skill, $p$, is uniformly distributed between 1 and 2.
    \item students are randomly allocated a good college ($\ec = 1+\epsilon$) and a mediocre college ($\ec = 1$) by coin flip.
    \item grad school has environment factor of $\eg = g$.
    \item grad school can only admit 1/2 of all the students
\end{itemize}

Then, the grad school admits $\frac{R}{2}$ of the students from mediocre college, where \[ R = \begin{cases} \frac{1}{1+\epsilon} &\text{ if grad school ranks students by current skill}\\
    \frac{1+g}{1+\epsilon+g} &\text{ if grad school ranks students by future skill}\\
    1 &\text{ if grad school ranks students by $p$ (``equality of opportunity'')}
    \end{cases}\]

    Note that as $g\to \infty$, $\frac{1+g}{ 1+\epsilon+g} \to 1$. Thus it can be said that future skill interpolates between current skill and ``equality of opportunity''.
\end{example}

\pagebreak

Notes for Feb 26th
\begin{itemize}
    \item Rooney rule: https://arxiv.org/pdf/1801.03533.pdf

    Applying this to future achievement?
    \item Answering an engineering question, say you have data.
    \item Do admissions committees already appreciate this point about future achievement / correcting for environment confounder?

    Yes -Christian. e.g. saying that student is `maxed out'.

    but there are always professors who say that this is only for diversity and not quality.

    \item future achievement interacts with selection effect. Should you give more opportunity to high schools that select for future achievement as well?

    \item if there are multiple schools and all schools rank students the same, then admissions policy of one school to improve overall welfare (e.g. a student who would not have been admitted by any of the other good schools)
\end{itemize}

Model to discuss for Feb 26th meeting:
\begin{enumerate}
    \item We could model current skill $\sc$ like in Nikhil's paper. i.e. There are $K$ observed features and $\theta_k = \sc + \epsilon_k$, where $\epsilon_k$ is Gaussian noise.
    \item Or something more general: \begin{equation}
        \theta = \ec \cdot v + \epsilon
    \end{equation}. In the above model $v$ would be the $K$-dim all ones vector, and $\epsilon$ is a $K$-dim vector of Gaussian noise.
    \item Yet another even more general model: $\theta = f(\sc, \ec, p)$. e.g.
    \begin{equation}
        \theta = \sc \cdot v_s + \ec \cdot v_e + p \cdot v_p + \epsilon
    \end{equation}
    I'm not sure it makes sense to have $p$ in there. Possibly the features should be independent of $p$ conditioning on $\sc$, i.e. SAT score should be independent of ability to learn conditioning on current skill.

    It is possible that the environment $\ec$ affects the features, even after conditioning on current skill? e.g. more prestigious college means more famous professors who write more impressive rec letters?
    \item If we model the skill acquisition process as:
    \begin{equation}
        \sc = \sn+g(\ec\cdot p \cdot t)
    \end{equation}
    Then we could have:
    \begin{equation}
        \theta = \sc \cdot v_s + \ec \cdot v_e  + \epsilon =  (\sn+g(\ec\cdot p \cdot t))v_s +  \ec \cdot v_e  + \epsilon =
    \end{equation}
    But then under this model, it is clear that any feature is equally informative about the current skill $\sc$ as they are about the ability to learn $\ec$
\end{enumerate}

Looking at distributions of $p$ and how that affects the optimal admissions policy
\begin{itemize}
    \item If we knew the current skill $\sc$, initial skill $\sn$ and the environmental factor $\ec$, we can directly infer $p$ (assuming $t=1$):
    \[ p = \frac{g^{-1}(\sc - \sn)}{\ec} \]
    \item is it more interesting when $\ec$ is unknown and must be somehow inferred from average population statistics? e.g. $g$ is linear and \[\widehat{\ec} = \frac{\E[\sc] - \E[\sn]}{\E[p]},\] where $\E$ is over the applicant pool.
\end{itemize}

Meetings notes
\begin{enumerate}
    \item Questions that are worth clarifying: Resolving the tension between diversity and achievement?

    What's a possible theorem statement?
    E.g. You admit more students from a disadvantaged background under the future achievement model.
    But this depends on the distribution of $p$ (how $p$ is concentrated in different environments?, the tail matters)
    Under some conditions, you could still be admitting people based on current skill primarily?

    imperfect learning of p and of current skill.

    Future achievement model tells you you should weight certain features more.

    prestigious college feature could be a downweight?

    The point has been made that features must be considered in their context (Nikhil's paper). Better to focus on the future achievement aspect.
    Also the point that what you're predicting as an objective is important.

    A different perspective on why diversity is important.
    \item literature review of models for admissions.
    \item Like in Nikhil's paper, could assume you have a model to learn single dimensional current skill from all available features. Features are a function of $\ec, \sc, p$
    \item The features for predicting current skill could be different from those for predicting future skill.
    \item $\sc = \sn+g(\ec\cdot p \cdot t)$, where $t$ is time. and g could be linear or have decreasing marginal returns.
\end{enumerate}

\begin{itemize}
    \item Students apply for admission with observable traits $(\ec, \sc)$, where $\ec$ is the previous academic environment and $\sc$ is the current skill level. They have unobservable trait, $p$, which is an innate propensity for skill improvement. $(\ec,\sc,p)$ are distributed according to population distribution $\calP$.
    \lnote{Could have different distributions for an advantaged group and a disadvantaged group.}
    \item Current skill level is a function of $\ec$, $p$, and initial skill, $\sn$ e.g.,
    \begin{equation}
        \sc =h(\ec, p, \sn) = \ec\cdot p\cdot \sn
    \end{equation}
    \lnote{Not sure about this functional form. Does it model effects that we're interested in?}
    \item The graduate school has environmental factor $\eg$.
    \item The admissions committee has a model for a student's future achievement, $\sg$:
    \begin{equation}
       \sg = h(\eg, p, \sc) = \eg \cdot p \cdot \sc.
    \end{equation}
    \item A naive goal is to admit a class of students with the highest current skill. Suppose $\rho$ is the proportion of the applicant pool that the committee wants to admit. Let $\calF$ be a class of functions that map the observable traits $(\ec, \sc)$ to an admissions outcome $f(\ec, \sc) \in \{0,1\}$.

    The admissions committee solves the problem:
    \begin{equation}
        \max_{f\in \F: \E_{\calP}[f] = \rho} \E_{\calP} \left[f(\ec, \sc)\cdot \sc \right]
    \end{equation}
    \item
   A less naive goal is to admit a class of students with the highest future achievement. The admissions committee solves the problem:
    \begin{equation}
        \max_{f\in \F: \E_{\calP}[f] = \rho} \E_{\calP} \left[f(\ec, \sc)\cdot h(\eg, p, \sc)\right]
    \end{equation}
\end{itemize}




\section{Two skills model}

\lnote{High level message? Changing the relative importance of metrics/features affects student effort in different activities. The effort has different payoffs for students in different environments. This would be different argument from the model in Garg et al 2020 and Emelianov et al 2020, which is based on the amount of information in each feature, for perhaps a similar high-level point.}

This model is based on \citet{calsamiglia09decent}, which extends earlier models on effort and equality of opportunity (e.g. John Roemer's work).
\begin{itemize}
    \item 2 students, $\A$ and $\B$.
    \item 2 skills/activities: $T$ (Testing) and $R$ (Research).
    \item Irrelevant characteristics for each activity (e.g. school resources for undergrad research): $(b^\A_T,b^\A_R), (b^\B_T,b^\B_R)$
    \item Relevant characteristics for each activity (e.g. creativity):  $(r^\A_T,r^\A_R), (r^\B_T,r^\B_R)$
    \item Effort level chosen by student: $(e^\A_T,e^\A_R), (e^\B_T,e^\B_R)$
    \item Performance in each activity. For both students: \[p_T = b_T r_T \sqrt{e_T}, ~p_R = b_R r_R \sqrt{e_R}, \]
    which exhibits decreasing marginal returns to effort.
    \lnote{In the original model, the innate ability for each skill only affects the performance in that skill. Suppose it's also possible that there are two innate abilities, both of which affect both performances in different ways?} \nikhil{Yes, or it might be worth eventually trying to get the full generality of any number of abilities map to the skills arbitrarily.}

    \nikhil{Related -- I've struggled with this in the past: I don't think the terms "innate ability," "effort," and "skill" quite capture what we mean here. For ex, grad schools admit for estimated research \textit{potential}, which weakly depends on past \textit{preparation}. I don't yet have a good recommendation.}

    \item Cost of effort: $(e_T+e_R)^2$.
    Marginal cost of effort increases in the effort expended for both activities, modeling the trade-off.
    \item Welfare gains to student. Student chooses effort level in 2 activities to maximize this objective:
    \begin{equation*}
        \alpha p_T + (1-\alpha)p_R - (e_T+e_R)^2
    \end{equation*}
    $\alpha$ is relative weight of the 2 activities in the admissions decision.

An admissions policy that is `consistent' with this objective is: with probability $\alpha$, the student is admitted with probability $p_T$ (based on testing performance), and with probability $1-\alpha$, the student is admitted with probability $p_R$ (based on research performance. The student chooses effort to maximize their overall probability of admission minus the cost of effort.

    \nikhil{Getting the admissions policy "right" is I think central to the work. We'll need a convincing model of: "How do admissions committees where different skills matter (differently for different committee members(?)) work?" In particular, I think if we're not careful, we'll have just really solved a single-dimensional problem with 1 extra layer of how different measures map to that single merit dimension.}


\end{itemize}

The main result from \citet{calsamiglia09decent} is the following:
\begin{proposition}[Informal]
Students $\A$ and $\B$ who differ \emph{only} in irrelevant characteristics can have different welfare gains under this model. Affirmative action (i.e. bumping up the performance of the student with disadvantaged irrelevant characteristics) still results in unequal welfare gains.
\end{proposition}

\begin{proposition}
`Equalizing rewards to effort' results in equal welfare gains, but requires knowledge of the irrelevant characteristics.
\end{proposition}


==> related.tex <==
\subsection*{Related work}
Our work sits at the intersection of work in two communities,
\textit{strategic classification} and \textit{fair machine learning} in computer science, and \textit{contests} and \textit{effort} in economics. %\nikhil{3 audiences -- classification, FATE, economics}
%
In developing a framework for strategic ranking, we primarily contrast with the main findings of the \textit{strategic classification} literature, demonstrating how a simple change from the classification to the ranking setting changes many insights. Our analyses are also motivated by recent work considering equity in allocation and ranking problems. In pursuit of these questions, our theoretical framework borrows from the economics literature on \textit{contests}, in which agents expend effort to obtain a reward that is a function of their relative performance across agents.

%\footnote{equivalently, binary classification to constrained binary classification holding constant the number of positive labels}

%\nikhil{From Christian -- less defending of work from econ audience, speak more to CS audience and be honest about what we get from the econ audience. Maybe be even more explicit about it, relate to the FATE community more}


% Our work is at the intersection of two literatures that consider these effects.  As in ranking contests \nikhil{wc?}, in our model agents are further incentivized by competition from other agents. We show how the two effects interact, and how the challenge of accurately ranking agents is complicated by needing to incentivize productive effort.

\parbold{Strategic classification} As in strategic classification~\cite{Hardt:2016:SC,miller2020strategic}, we consider the challenge an institution faces when deploying a classifier that applicants can game; a naive classifier that does not factor in the resulting distribution shifts would be inaccurate. Unlike strategic classification, which considers the manipulation of observable features to be unproductive from the institution's perspective, our model of efforts stipulates that the school prefers higher effort levels as they give rise to higher scores.  We follow the line of work considering the design of reward functions that further incentivize agent effort on productive tasks~\cite{kleinberg18investeffort}.

We in particular draw inspiration from and compare to several recent directions in the strategic classification literature: with multiple agents, when a classifier may be random, and with fairness concerns.~\citet{haghtalab2020maximizing} and~\citet{alon2020multiagent} both study multi-agent strategic classification where the principal's goal is to incentiv{ize} %e
% 
agents to improve their features in a productive manner (as opposed to, e.g., cheating); in our setting, the different agents may have different initial features and cost functions, but also impose competitive pressures on each other. \citet{hu2019disparate} and \citet{Milli2019social} consider the (potentially heterogeneous) cost of strategic classification on applicants, as in equilibrium (due to the classifier's adjustment) they must exert extra effort to be admitted. In our model with disparate costs, a student from the disadvantaged group similarly must exert a greater effort to be admitted than a student from the advantaged group, and this effort differential worsens with increased competition. Finally, \citet{braverman2020role} study the role of randomized classifiers and noisy features in strategic classification, showing that a randomized classifier can prevent  undesirable strategic behavior {by an applicant}; they further show that \textit{after} applicants have responded to a randomized classifier, randomization is not a best response for the institution. It is also shown that noisy features can reduce disparate impact when there are two subpopulations with different costs of manipulation. In our setting, randomization (after applicants have been ranked) plays three roles: to prevent strategic behavior at the cost of other, less measurable beneficial features, to lessen competitive pressure, and to increase fairness in the presence of disparate costs. %In our setting, we find that using a randomized decision policy could be justified by social welfare objectives or when there is a unmeasurable attribute.

Like other strategic classification work, our work is further related to the prior economics literature on contract design, elaborated in \Cref{sec:multi-dim}. % \todo{other contract design}
%Most related is the work of


\parbold{Economics: Contests and modeling effort} Our theoretical analysis is similar to that in the literature on \textit{contests} in economics~\cite{barut1998symmetric}; e.g., our rank preservation result in \Cref{sec:equillemmas} reflects assortative allocation results in the literature under similar conditions. The field is too extensive to summarize here, so we refer the reader to surveys~\cite{corchon2007theory,fu2019contests} and discuss the works closest to ours.

\citet{bodoh2018college} develop a model with heterogeneous students endogenously choosing effort in an admissions game; they use the model to compare various affirmative action schemes. \citet{fang2020turning} find that increased competition (in form of either more contestants or more convex reward structure) decreases overall student effort. Most related is the line of work by~\citet{olszewski2016large,olszewski2019bid,olszewski2019pareto}. \citet{olszewski2019pareto} find that policies that ``pool'' individuals into tiers (as opposed to continuous ranks) can be Pareto improving for students; even those with decreased individual rewards would benefit from decreased competitive pressure. 

Our work departs from the contests literature through its focus on the questions most common in the strategic classification literature: while the contests literature primarily considers the efforts and resulting welfare of participants, we study how the design of the reward function $\lambda$ differentially affects the corresponding designer's utility, applicant welfare, and fairness metrics. In particular, when $\lambda$ is interpreted as a probability of admission, our designer faces tradeoffs with incentivizing overall effort and admitting the most skilled students (\Cref{sec:welfare}); with disparate access, the designer must further navigate trade-offs between fairness and inducing effort (\Cref{sec:environment}); with multiple score dimensions, the designer must ensure that applicants do not excessively game one dimension at the cost of the other (\Cref{sec:multi-dim}). Simultaneous to us, \citet{elkind2021contest} consider the effect of contest design on participant and designer welfare. 

Beyond the contests literature, our work connects to the economics literature on student effort and subsequent reward. We incorporate two well-studied rewards from effort: a signal of one's quality in a competition~\cite{spence1978job} (in our model, the incentive of students), and productive development of human capital~\cite{becker1973theory} (in our model, the goal of the school). Following \citet{roemer1998equality}, \citet{calsamiglia09decent} considers a model in which measurable performance in a competitive activity is a product of effort, a relevant characteristic (such as talent), and an irrelevant characteristic (such as environment); the work studies mechanisms to achieve global equality of opportunity---in which students' post-allocation welfare does not depend on irrelevant characteristics---when allocations are determined locally for each competitive activity, e.g., the NBA and college admissions.
% \todo{where does this go? Lydia is this that paper that you were looking at earlier?}
%  \lnote{Yes. I added a blurb. }
% \lnote{This would fall under the line of work on equality of opportunity, which formalized the concept of effort etc. }




\parbold{FATE in machine learning and MD4SG} Finally, we broadly connect to the Fairness, Accessibility/Accountability, Transparency, and Ethics (FATE) in machine learning \cite{Chouldechova2018TheFO} and the Mechanism Design for Social Good (MD4SG) literatures \cite{abebe2018mechanism}. Most relevant are works on fair ranking, constrained allocation, and admissions. The fair allocation literature also considers the allocation of (often indivisible) resources in a budgeted setting, with various fairness notions defined at the group or individual level~\cite{aziz2020developments,caifair2020,golz2019paradoxes,noriega2019active}---such as when one group due to external discrimination faces a disadvantage in features. Similarly, fair ranking works consider the distribution of ranking slots to agents who belong to various groups~\cite{mathioudakis2020affirmative,zehlike2017fa,zehlike2020reducing} or to items that each have a certain social utility \cite{tabibian2020design}. In both settings, the mechanism designer must balance allocation based on ``relevance'' with an appropriate fairness notion. Finally, the burgeoning mechanism design literature on fair admissions (and more generally, classification) considers the design of mechanisms that can counter historic and ongoing inequities~\cite{faenza2020impact,garg2020dropping,immorlica2019access,kannan2021best,liu2020disparate,Hu2018shortterm,Mouzannar2019socialequality,kannan2019downstream,liu2018delayed,rolf2020balancing,liu2021test}. In this work (and especially in \Cref{sec:environment}), we consider such effects as they interact with agents' strategic responses to the mechanism.

%Finally, our work is part of the burgeoning , which considers the design of mechanisms 
%Much of the fair allocation literature studies information acquisition policies by the school, without considering agents' strategic responses \cite{aziz2020developments}.~\citet{noriega2019active} and \citet{caifair2020}, for example, also consider various fairness notions in a budgeted setting, when the school can acquire additional information on applicants. 








%\todo{include citations to fair ML work in education/allocation in general, to the community that will read this paper} ~\cite{,} 

% \nikhil{include your works too here, Lydia!}

%\cite{liu2020disparate,Hu2018shortterm,Mouzannar2019socialequality,kannan2019downstream} dynamics of decision making and ramifications for fairness.
%
%\cite{liu2018delayed, rolf2020balancing} considered multiple objectives.
